Metaheuristics "In the Large"

Following decades of sustained improvement, metaheuristics are one of the great success stories of optimization research. However, in order for research in metaheuristics to avoid fragmentation and a lack of reproducibility, there is a pressing need for stronger scientific and computational infrastructure to support the development, analysis and comparison of new approaches. We argue that, via principled choice of infrastructure support, the field can pursue a higher level of scientific enquiry. We describe our vision and report on progress, showing how the adoption of common protocols for all metaheuristics can help liberate the potential of the field, easing the exploration of the design space of metaheuristics.

==> authors.tex <==
\author{Jerry Swan$^1a$, 
Steven Adr\ae nsen$^b$,  
Alexander E.\ I.\ Brownlee$^c$,
Colin G.\ Johnson$^d$,
Ahmed Kheiri$^e$, 
Faustyna Krawiec$^f$,
J.\ J.\ Merelo$^g$, 
Leandro L.\ Minku$^h$, 
Ender \"Ozcan$^i$, 
Gisele L.\ Pappa$^j$, 
Pablo Garc\'ia-S\'anchez$^k$,
Kenneth S\"orensen$^l$, 
Stefan Vo{\ss}$^m$,
Markus Wagner$^n$, 
David R.\ White$^o$ \\
\vspace{0.5cm}
$^1$ Corresponding author.\\
$^a$ jerry.swan@york.ac.uk. University of York, Heslington, York YO10 5DD, UK.\\
$^b$ st.adriaensen@gmail.com.  Vrije Universiteit Brussel, Pleinlaan 2 1050, Brussel, NL.\\
$^c$ alexander.brownlee@stir.ac.uk. University of Stirling, Stirling, FK9 4LA. UK.\\
$^d$ c.g.Johnson@kent.ac.uk. University of Kent, Canterbury, CT2 7NF, UK.\\
$^e$ a.kheiri@lancaster.ac.uk. Lancaster University, Lancaster, LA1 4YW, UK.\\
$^f$ fmk31@cam.ac.uk. University of Cambridge, Cambridge, CB3 0FD, UK.\\
$^g$ jmerelo@kal-el.ugr.es. Universidad de Granada, Granada, ES.\\
$^h$ l.l.minku@cs.bham.ac.uk. University of Birmingham, Birmingham, B15 2TT, UK.\\
$^i$ ender.ozcan@nottingham.ac.uk. University of Nottingham, Nottingham, NG8 1BB, UK.\\
$^j$ glpappa@dcc.ufmg.br. Universidade Federal de Minas Gerais, Belo Horizonte, 31270-010, BR.\\
$^k$ pablogarcia@ugr.es. University of Granada, 18071, Granada, Spain.\\
$^l$ kenneth.sorensen@uantwerpen.be. Universiteit Antwerpen, Prinsstraat 13, 2000 Antwerp, NL.\\
$^m$ stefan.voss@hamburg.de. Universit\"at Hamburg, 20146 Hamburg. DE.\\
$^n$ markus.wagner@adelaide.edu.au. University of Adelaide, Adelaide, SA 5005, AU.\\
$^o$ d.r.white@sheffield.ac.uk. University of Sheffield, Sheffield S10 2TN, UK.
}

